Sample Efficient Demonstration Selection for In-Context Learning

The in-context learning paradigm with LLMs has been instrumental in advancing a wide range of natural language processing tasks. The selection of few-shot examples (exemplars / demonstration samples) is essential for constructing effective prompts under context-length budget constraints. In this paper, we formulate the exemplar selection task as a top-m best arms identification problem. A key challenge in this setup is the exponentially large number of arms that need to be evaluated to identify the m-best arms. We propose CASE (Challenger Arm Sampling for Exemplar selection), a novel sample-efficient selective exploration strategy that maintains a shortlist of "challenger" arms, which are current candidates for the top-m arms. In each iteration, only one of the arms from this shortlist or the current topm set is pulled, thereby reducing sample complexity and, consequently, the number of LLM evaluations. Furthermore, we model the scores of exemplar subsets (arms) using a parameterized linear scoring function, leading to stochastic linear bandits setting. CASE achieves remarkable efficiency gains of up to 7x speedup in runtime while requiring 7x fewer LLM calls (87% reduction) without sacrificing performance compared to state-of-the-art exemplar selection methods. We release our code and data at https://github.com/kiranpurohit/CASE

==> 1_intoduction.tex <==
\section{Introduction}
\label{sec:intro}

% \color{blue}
% In-context learning can be used to effectively solve difficult NLP problems like reasoning tasks, without re-training large language models. However, standard exemplar selection techniques are ineffective on these problems due to low-robustness of the resulting learner (Venkatesh: give reasons). \\
% In-context exemplar selection is a search problem over an exponentially large set of subsets, which is infeasible through brute force methods due to the computationally expensive LLM calls for evaluating each subset.\\
% A principled approach to solving this problem can be formulated as approximating the scores of \textbf{high-scoring exemplar subsets} using a linear function of the features of exemplars.\\
% We formulated this problem of jointly finding the high-scoring exemplar subsets, and also estimating their score as a problem of pure exploration.\\
% The key challenge is to design an algorithm for finding top-$m$ subsets in the stochastic linear bandits setting, without explicitly sampling all the arms.\\
% We propose a novel challenger sampling-based algorithm for the above problem.
% \color{black}
% $N(\mu, \sigma)=\frac{1}{\sqrt{2 \pi} \sigma} (x-\mu)^2 2\sigma^2$

% Many data-centric AI application's e.g. efficient training\citep{}, efficient evaluation \citep{}, responsible AI \citep{}, require a data subset selection algorithm in the background. \\
Recent advances in Natural Language Processing (NLP) tasks have been fuelled by Large Language Models (LLMs) \citep{brown2020gpt3,gpt3incontext,openai2023gpt4}. Such models exhibit emergent capabilities like in-context learning (ICL) \citep{gpt3incontext}, which entails learning from few-shot samples (input-output pairs) \citep{few_shot,li2023fewshot} along with Chain-of-Thought (COT) rationale explaining the reasoning process to the LLM.
% For complex reasoning tasks like numerical reasoning based Financial Question Answering (QA) \citep{chen2022finqa,tabmwp}, commonsense and compositional reasoning based QA \citep{strategy_qa} a Chain-of-Thought (COT) rationale explaining the reasoning process is provided with each input-output example. 
This triplet of (input, rationale, output) is termed as \textit{exemplar} and the rationale is particularly critical for complex reasoning tasks like multistep reasoning based QA \citep{strategy_qa,chen2022finqa,tabmwp}. We term the paradigm of performing of ICL with rationale augmented examples (exemplars) as In-Context Reasoning (ICR). A principled selection of the few-shot exemplars is a challenging problem, as ICL is sensitive to the quality of the exemplars provided \citep{lu-etal-2022-fantastically,zhao2021calibrate}.

\begin{figure*}
    \centering
    \includegraphics[width=0.92\linewidth]{figures/CASE_final-cropped.pdf}
    \caption{An overview of \static{} for selection of top-m exemplar subsets}
    \label{fig:enter-label}
\end{figure*}
% In-context learning methods have shown promise in many complex real-world NLP tasks e.g. complex question answering \citep{},  numerical reasoning \citep{}, reasoning with tabular datasets \citep{}, etc.
% Many of these applications require careful selection of a small number of in-context examples, from a "training set", that optimally describe the intention of the task.
The majority of existing approaches for exemplar selection report heuristic or trial and error based efforts \cite{complex_cot,few_shot} except for a few approaches that attempt to tackle the problem in a principled manner \cite{xiong2024dqlore}. The exemplars selected for ICR can be categorized into \textit{task-level} where a static set of exemplars representative of the task are selected and used for inference and \textit{instance-level} exemplars where exemplars are selected dynamically for each test instance during inference. Instance level selection approaches typically employ similarity \citep{rubin-etal-2022-learning,xiong2024dqlore} and diversity based measures \citep{ye-etal-2023-complementary} to select the most suited exemplars from the training pool for each test instance, incurring overhead during inference. Additionally, instance-level selection approaches do not consider the positive and negative interactions between the exemplars, as they select each exemplar independently. Selecting a static set of exemplars for the task (task-level) not only obviates inference time overhead but also enables prompt caching that entails reusing key-value (KV) attention states \cite{gim2024promptcachemodularattention} for the prompts. Hence, in this  work, we propose a principled approach for task-level exemplar selection. The closest work that proposes a task-level exemplar approach is LENS \cite{li2023finding} which requires expensive computations as each exemplar in the training pool is valued using an informativeness measure that relies on calling a LLM over multiple iterations. Moreover, LENS relies on confidence measure from LLM rendering it difficult to extend to black-box LLMs and also does not model interactions between exemplars.  We propose to implicitly model the interactions between the exemplars by scoring exemplar subsets as a whole rather than scoring them independently.

One of the challenges towards proposing a principled solution is that the actual mechanism of in-context learning is not well understood.
Recent studies towards building theoretically grounded models for in-context learning \citep{zhang2023trainedtransformerslearnlinear} apply primarily to linear functions/models and linear transformers.
Hence, for a principled efficient selection of exemplars, we need a surrogate model for modelling the goodness of an in-context learning procedure. 

% Another important challenge is to solve the dual problem of learning the parameters of the model and selecting the best subset of training examples which maximize the accuracy.
We formulate the selection of top-$m$ exemplar subsets as the problem of pure exploration \citep{LUCB} in the stochastic linear bandit setting \citep{reda2021top}. 
Specifically, we explore the problem of identification of top-$m$ arms \citep{reda2021top}. While several uniform sampling algorithms for top-$m$ arms identification exist, \cite{pmlr-v54-chen17a,pmlr-v30-Kaufmann13} they do not focus on efficiency. While the GIFA framework \citep{reda2021top} proposed an efficient gap-index based top-$m$ arms identification algorithm with reduced sample complexity. However, the computation of \textit{challenger arm} (current candidates for top-$m$ arms), requires large number of gap-index computations due to the large space of candidate arms that are currently not the top-$m$ arms. 

In this work, we propose \static{} (\textbf{C}hallenger \textbf{A}rm Sampling for Exemplar Selection) where we propose a principled sampling of challenger arms to form a shortlist challenger set, pruning the space of possible candidate arms. This leads to further reduced sample complexity, gap-index computations and efficient runtime of the one-time exemplar selection.


\textbf{Contributions:}
\begin{itemize}
    \item We propose a novel and principled gap index, MAB based approach for task level exemplar selection. Our contribution primarily lies in principled challenger arm sampling to prune the search space, which renders the process highly efficient compared to state-of-the-art MAB frameworks and other subset, exemplar selection approaches. 

\item We provide theoretical bounds for sample complexity and the regret bound for \static{}.
    \item We perform extensive experiments on diverse tasks that require complex reasoning and observe that \static{} is sample efficient and yields high gains compared to other state-of-the-art exemplar selection approaches.
\end{itemize}




==> 3_methods_old.tex <==
\section{\static{}: Challenger Arm Sampling-based Exploration for Exemplar-subset Selection}

In the in-context learning paradigm, the problem of constructing an optimal prompt for a given task is formulated as an \textit{exemplar subset selection} problem (section \ref{sec:formulation}).
In section \ref{sec:top-m-arm}, this problem is modeled as a top-$m$ arm selection problem in linear stochastic bandits \citep{kalyanakrishnan2010efficient,reda2021top}, where we use a linear function as a proxy for the loss of a given arm (prompt).
Section \ref{sec:algo}, proposes a novel \textit{selective exploration}-based algorithm, (conceptually close to the SETC \citep{lattimore2020bandit}), which samples and stores the ``challenger arms'' (arms which can potentially be in the top-$m$ set \citep{reda2021top}). This reduces the computational overhead of evaluating every possible arm in each iteration.
Section \ref{sec:convergence} outlines a probabilistic guarantee on the top-$m$ regret, which measures the suboptimality of the top-$m$ arm selection.


\subsection{Exemplar-subset Selection for In-Context Reasoning}
\label{sec:formulation}

\color{red}
% use $u,v$ for exemplars (in-context examples) and $u',v'$ for validation exemplars.\\
use $\mathbf{x}$ and $y$ for denoting feature vectors of arms.\\
We are using $n,n'$ for training and validation set size.
\color{black}

In-context learning (ICL) allows LLMs to be used for new tasks, e.g. financial question answering\citep{chen2022finqa}, numerical reasoning \citep{tabmwp} etc. by leveraging a few demonstration examples of the task without training or parameter fine-tuning.
In this process, the LLM is provided with a prompt (P) containing input-output pairs with rationales, called \textit{exemplars}, which demonstrates the task to the LLM. We term the paradigm of ICL with rationales as In-Context Reasoning (ICR) for the rest of the paper.
Let $\cX = \{u_i, v_i\}^{n}_{i=1} $ be the set of all $n$ training examples (potential exemplars) illustrating the task and $u_{test}$ be a test input.
The goal is to predict the test output $v_{test}$. 
Let $S\subseteq\cX$ denote a subset of $k$ exemplars to be used for prediction of $u_{test}$. 
The prompt $P$ can be constructed as:
%\begin{equation}
 $ P = [S, u_{test}] = [(u_{i_1}, v_{i_1}), . . . , (u_{i_k}, v_{i_k}), u_{test}] $ 
 % \label{eq:prompt}
% \end{equation}

Alternatively,  an approach $\psi(S_1,..., S_m, u_{test})$ that uses multiple high-scoring subsets $S_1,..., S_m$  and a test input $u_{test}$ to generate a prompt $P$ that is expected to improve the overall performance or robustness of ICR compared to prompts generated using a single exemplar subset. 
Also, let $f$ denote the response generator function for a given LLM. 
% \begin{equation}
  Hence, $ f(P) = \cG\left(\bP_{LLM}(r|P)\right)$ % \label{eq:LLM}
% \end{equation}
where, $\cG$ denotes the decoding mechanism of the LLM which can be used to sample response $r$ from the probability distribution $\bP_{LLM}$.
Let $\delta$ denote the post-processing step applied to the LLM-generated response, $f(P)$ such as Regex or self-consistency \cite{wang2022self}, in order to extract the task-specific output $\hat{v}_{test}$.
% Commonly used post-processing strategies include regular-expression matching ($\delta_{regex}$) and  self-consistency ($\delta_{SC}$) \cite{wang2022self} based strategies.

% The problem of \textit{in-context reasoning} (ICR) is especially challenging because the relationship between the exemplars and the LLMs ability to perform a multi-step reasoning task on a given test example is not clear.
% prompt formulators can be used to improve the effectiveness of ICR tasks.
% A prompt formulator $\psi(S_1,..., S_l, u_{test})$ uses multiple high-scoring subsets $S_1,..., S_l$  and a test input $u_{test}$ to generate a prompt $P$ that is expected to improve the overall performance or robustness of ICR compared to prompts generated using a single exemplar subset. 
% For example, we use a similarity-based prompt formulator $\psi_{KNN}$ and a diversity-based prompt formulator $\psi_{MMR}$ or $\psi$ selects the subset with the lowest validation loss (the details are described in section \ref{sec:experiments}). 
Hence, the entire output generation process can be described as:
\begin{equation}
\hat{v}_{test} = \delta(f(P)), \mbox{ where } P=\psi(S_1,...,S_m, u_{test}) %= \delta(f([S_,x_{test}])) 
\label{eq:predictive-model_static}
\end{equation}
\color{black}
Let $\cV$ be the set of $n'$ validation examples $\{u'_i, v'_i\}^{n'}_{i=1}$. 
% We define the validation accuracy for a  prompt $P$ as:
% \begin{equation}
%    A(P, \cV) = \frac{1}{n'} \sum_{i=1}^{n'} \ind(v'_i = \delta(f(\psi(S_1, ... , S_l, u'_i))) \label{eq:loss}
% \end{equation}
In exemplar selection, we are interested in finding an optimal subset of training examples $S^* \subseteq \cX$ which maximizes the validation accuracy ($A(P,\cV)$). However, in the present setup, we are interested in finding a set $U=\{ S_1, ...., S_m \}$ of subsets such that the corresponding prompt $P$ generated by $\psi$ yields optimal performance such that $U^* = \argmax_{U={S_1,...,S_m}} A(P,\cV)$
% \begin{equation}
%     U^* = \argmax_{U={S_1,...,S_l}} A(P,\cV) \label{eq:exemplar-select}
% \end{equation}

\subsection{Top-$m$ Arm Selection formulation for Prompt Generation}
\label{sec:top-m-arm}
\color{red}
There are two main challenges in efficiently solving the exemplar subset selection problem (Eq \ref{eq:exemplar-select}):
(1) the set of all exemplar subsets $\cS$ can be very large leading to prohibitive time-complexity. For instance, $n=5000$ training examples, and a prompt size of $k=5$ examples lead to $C^5_{5000}$ (approximately $2.5 *10^{16}$) exemplar subsets. 
% This task is computationally demanding due to the need for LLM inference calls to evaluate all combinations to find the optimal subset of exemplars. 
(2) a naive calculation of loss (Eq \ref{eq:loss}) for each exemplar subset $S$ involves $m$ calls ($m\sim 1000$) to the LLM, which can be expensive (both computationally and financially). We address the first issue in section \ref{sec:staticselection}. We propose to address the second issue by building a \textit{scoring function} ($\sigma$) for the subsets $S\in \cS$, which can be used to calculate the top-$l$ subsets without making calls to the LLM.


% Let $\sigma(S)$ denote the proposed \textit{scoring function} for the subset $S$. 
Intuitively, given a subset $S$, the scoring function $\sigma(S)$ should model the validation loss of an exemplar subset, $L(\psi,\{S\},\cV)$, since they are expected to generate identical rankings.
Hence, we propose that $\sigma$ should incorporate the relationship between the exemplar's question $x_i$ and the validation example's question $u_j\in \cV$.
%, which is crucial for effectively approximating the loss $L(S,\cV)$.
In this work, we capture the relationship using a similarity score, $E_{ij} = \frac{\phi(x_i)^T\phi(u_j)}{\|\phi(x_i)\|\|\phi(u_j)\|} $, where $\phi(x)$ is the feature encoding of a smaller transformer model, e.g. BERT. 
%, thus making the scoring function efficient to calculate. 
% We define BERT similarity-based feature as $E_{ij} = \frac{\phi(x_i)^T\phi(u_j)}{\|\phi(x_i)\|\|\phi(u_j)\|} $ where $\phi(x)$ is the pre-trained BERT embedding of example $x$. 
We model score as linear function of the similarity features $E_{ij}$ of exemplars $x_i$ in the subset $S$:
\begin{align}
 \sigma(\Vec{\alpha}, S) = \frac{1}{m} \sum_{j=1}^m \sum_{i=1}^n \alpha_i \ind(x_i\in S) E_{ij}
\end{align}
Here, $\alpha_i$ denotes the $i$-th exemplar's contribution to the scoring function. We dynamically estimate $\alpha_i$ to fit the top-$l$ (lowest loss) exemplar subsets in $\cS$. Section \ref{sec:staticselection} describes the details of the algorithm.

Note that since $\alpha_i$'s can be negative, they can be learned to implicitly estimate both positive and negative correlations between training exemplars $x_i$ and $x_j$, according to signs of $\alpha_i$ and $\alpha_j$.
Also, note the above equation can be written as $ \sum_{i=1}^n \alpha_i \ind(x_i\in S) e_i$, where $e_i=\frac{1}{m} \sum_{j=1}^m E_{ij}$, which indicates that only aggregate effect of exemplars in validation set is modeled by $\sigma$.
Finally, training exemplars in ICL can be thought of as representing different ``distinguishable" solution ``concepts'' of tasks (see e.g. \cite{xie2021explanation}). 
For instance, consider the exemplars selected by \static{} for the AQUARAT dataset (Table \ref{tab:exemplar_qualitative_aquarat}) can be identified with concepts like \textit{Proportionality}, \textit{Series}, \textit{Kinematics}, and \textit{Interest}.
Since the final scoring function is trained to fit the top-$l$ exemplar subsets resulting in low loss, the resultant $\alpha_i$'s can be thought of as implicitly representing the important concepts needed for effectively predicting the correct label (hence resulting in low loss).
Unfortunately, since $\alpha_i$'s can be both positive and negative, their magnitudes are not directly interpretable as importance scores for the concepts.
Unlike existing works e.g. \cite{li2023finding, xu2024misconfidence}, we do not use probability scores for tokens provided by LLMs in our scoring function, as these scores are not directly related to the predictive task. 
\color{black}

We formulate the task of selecting exemplar subsets as the top-$m$ arms identification problem in stochastic linear bandits setting.
The top-$m$ arms identification problem involves identifying the set of m best arms ($S_m*=\{1,2..m\}$) with the largest means from the set of K arms, such that  $\rho_1\ge\rho_2...\ge\rho_m>\rho_{m+1}$ where $\rho_i$ refers to the actual mean of the arm $i$. The set $S_m^c = \{1...K\} \setminus S_m^*$ is the set of $K-m$ worst arms.

We propose \static{} a gap-index focused efficient algorithm building upon the existing GIFA framework \cite{reda2021top}.
The primary idea in \static{} is to estimate in each round t, a set of current top-$m$ arms $U_t$, determine the two most ambiguous arms namely $b_t \in U_t$ which is an estimate of m-best arm and a challenger arm $s_t \notin U_t$ which can be seen as a potential m-best arm that has been miscalculated. The challenger arm $s_t$ has the largest gap to $b_t$, that implies 

\subsection{\static{}: Challenger-arm sampling-based top-$m$ arm selection algorithm}
\label{sec:algo}

\color{blue}
$N_t$ ensure that a pulled arm is remembered unless there are $m'$ better arms already being remembered.\\
$B_t(i,j):$ gap index between arms $i$ and $j$ (positive if $i$ is better arm, or if $i$ is worse than $j$ but not by more than confidence between $i$ and $j$ which is $W_t(i,j)$)
\color{black}


\color{blue}
Here we say that the exploration is selective since we discriminate between the elements in the $N_t$ set and the $(U_t\cup N_t)^c$ set. All elements in the $N_t$ set are evaluated in every iteration as possible challenger, whereas only a uniform sample from 
\color{black}

The structure of \static{} is shown in Algorithm \ref{algo:static_subsets}. The set of top-m subsets (arms) $U$ is initialized to a random set sampled from $\cS$. The parameters for the linear model are sampled from a unit-Gaussian distribution. Then we compute the 

\begin{algorithm}[!t]
  \SetAlgoLined
 \small
 \caption{\static{} }
 \label{algo:static_subsets}
 % \color{blue}
 \textbf{Input:} $\cX$: set of all training examples (potential exemplars), $k$: the number of exemplars in a prompt\\
 Let $\cS:$ set of all subsets of size $k$ of potential exemplars, $a\in \cS$ denotes an arm, which is a subset of $k$-exemplars \\ 
 %$K \subseteq \cS$: All arms , $E_a, a\in[K]$: Input features for arms\\
  \textbf{Initialize:}   $U_0 \leftarrow$ set of random $m$ arms from $\cS$;  $t \leftarrow 1$; $\Vec{\alpha}_{1} \leftarrow \cN(0,1)$     %\Comment{$Vec{\alpha}_{1}$ from a gaussian } \\
  \\
   \textbf{Define:} $ U_t$: set of currently estimated top-$m$ arms, $N_t$: set of currently estimated next best-$m'$ arms., $b_t$: the most ambiguous arm from $U_t$,  $s_t$: the most ambiguous sampled arm from $N_t$
   
 \Comment{Stopping criterion}\\
\While{$B_t(s_t,b_t) \le \epsilon$ }  { 
           % \rho(\hat{\alpha_{t-1}^{\lambda}},s_{t-1}) \ge \rho(\hat{\alpha_{t-1}^{\lambda}},b_{t-1}
            \Comment{Construct $U_t$ from $U_{t-1}$ and $N_{t-1}$} \\
            $n_{t} = \argmin_{a\in U_{t-1}} \hat{\rho}_{t}(a) $\\
            $c_{t} = \argmax_{a\in N_{t-1}} \hat{\rho}_{t}(a) $\\
           \If{
           $\hat\rho_{t}(c_{t}) \ge \hat\rho_{t}(n_{t}) $ }
           {
            $U_t,N_t \gets \mbox{swap}(n_t,c_t)$ from $U_{t-1},N_{t-1}$         
           }
           
        \Comment{Construct $N_t$ from updated $N_{t}$ and sampling from  $U_t^c$} \\
        % $Q_t \leftarrow K\setminus U_{t}$
        $M_t \leftarrow s'\sim_{m'} U_t^c$ 
         
        $N_t \leftarrow \mbox{top}_{m'}(M_t \cup N_{t}; \hat{\rho}_{(t-1)})$

        \Comment{Calculate revised stopping criteria}\\
        $b_{t+1} = \argmax_{b\in U_t} \max_{s\in N_t} \left[ B_t(s,b) = \hat{\rho}_t(s) - \hat{\rho}_t(b) + W_t(s,b) \right]  $ \\
        $s_{t+1} =  \argmax_{s\in N_t} \left[ B_t(s,b_{t+1}) = \hat{\rho}_t(s) - \hat{\rho}_t(b_t) + W_t(s,b_{t+1}) \right]  $ 

        \Comment{pulling arm} \\
        $a_{t+1} \leftarrow$ selection\_rule$(U_t,N_t)$ \\
        $r_{t+1} \leftarrow \rho(\hat{\alpha}_{t}, a_t) + \eta_t$

        \Comment{Update the model}\\
        $\hat{V}_{t+1}^{\lambda} = \lambda I_N + \sum_{l=1}^{t+1} N_{a_l}E_{a_l} E_{a_l}^T$ \Comment{$\lambda$ regularized design matrix}\\
         $\hat{\alpha}_{t+1}^{\lambda}=(\hat{V}_{t+1}^{\lambda})^{-1}(\sum_{l=1}^{t+1} r_l E_{a_l})$ \Comment{Least-squares estimate}\\
         
        $t \gets t+1$
   } 
   
 \textbf{Output:}
 $U_T$: Set of $m$ arms from $K$ which have the highest reward 
\color{black}
\end{algorithm} 



Estimated mean:

\begin{equation}
 \hat\rho(\Vec{\alpha}, S) = \frac{1}{n'} \sum_{j=1}^{n'} \sum_{i=1}^n \hat\alpha_i \ind(x_i\in S) E_{ij} = \sum_{i=1}^n \alpha_i \ind(x_i\in S) \mathbf{E}_{i}
 \label{eq:reward}
\end{equation}

where $\mathbf{E}_{i} = \frac{1}{n'} \sum_{j=1}^{n'} E_{ij}$

%\subsection{ ChalSamp: Challenger Arm Sampling for Multi-Arm Bandit Based Exemplar Selection}
As stated earlier we cast the problem of task-level exemplar selection for 
% \begin{equation}
%     \cL(\Vec{\alpha};U_t,Q_t) = \sum_{s\in U_t}  ( A(s, \cV) - \rho(\Vec{\alpha},s))^2  +  \sum_{s' \sim Q_t}  ( A(s', \cV) -  \rho(\Vec{\alpha},s'))^2  
%     \label{eq:alphaloss}
%  \end{equation}






















% \begin{algorithm}[!httb]
%   \SetAlgoLined

%  \small
%  \caption{GIFA for ($\epsilon,\delta$)-PAC Top-$m$ }
%  \label{algo:gifa}
%  \small
%  % \color{blue}
%  \textbf{Input:} $K$ arms of means $\mu_1,\dots,\mu_K$; $\epsilon \geq 0$; $m \leq K$; $\delta \in (0,1)$\\
%   \textbf{Initialize:}  
%   \hspace{2mm}  $t \leftarrow 1$\\
  
   
% \While{$\neg$ stopping\_rule$((B_{i,j}(t))_{i,j\in[K]};\epsilon,t)$} {
        
%          $J(t) \leftarrow$ compute\_Jt$((B_{i,j}(t))_{i,j\in[K]}, (\hat{\mu}_i(t))_{i\in[K]})$ \Comment{$J(t)$: estimated m best arms at $t$}
        
         
%          $ b_t \leftarrow$ compute\_bt$(J(t),(B_{i,j}(t))_{i,j\in[K]})$ \Comment{$b_t$: estimated $m$-best arm at $t$} 
          
         
%          $ c_t\leftarrow \argmax_{a \not\in J(t)}B_{a,b_t}(t)$ \Comment{$c_t$: challenger to $b_t$ at $t$}


%          $ a_t \leftarrow$ selection\_rule$(b_t,c_t;\hat{V}_{t-1}^\lambda)$ \Comment{selecting and pulling arms}


%          $ r_t \leftarrow$ pulling$(a_t)$


%          Update design matrix $\hat{V}_t^\lambda$, means $(\hat{\mu}_i(t))_{i\in[K]}$


%          Update gap indices $(B_{i,j}(t+1))_{i,j\in[K]}$

        
%          $t \gets t+1$
%    } 

%    $\hat{S}^{T_\delta}_m \leftarrow J(T_\delta)$
   
%  \textbf{Output:}
%  $\hat{S}_m^{T_\delta}$ estimated $m$ $ \epsilon$-optimal arms at final time $T_\delta$
% \end{algorithm} 



% \begin{algorithm}[!httb]
%   \SetAlgoLined

%  \small
%  \caption{\static{} for ($\epsilon,\delta$)-PAC Top-$m$ }
%  \label{algo:explora_extension}
%  \small
%  % \color{blue}
%  \textbf{Input:} $\mu_1,\dots,\mu_K$: means of arms;  $\delta \in (0,1)$; $m \leq K$; $\epsilon \geq 0$ \\
%   \textbf{Initialize:}  
%   \hspace{2mm}  $t \leftarrow 1$\\
  
   
% \While{$\neg$ stopping\_rule$((B_{i,j}(t))_{i,j\in[K]};\epsilon,t)$} {
        
%          $J(t) \leftarrow$ compute\_Jt$((B_{i,j}(t))_{i,j\in[K]}, (\hat{\mu}_i(t))_{i\in[K]})$ \Comment{$J(t)$: estimated m best arms at $t$}
        
%          $M \leftarrow S'\sim (K \setminus J(t))$
         
%          $ b_t \leftarrow$ compute\_bt$(J(t),(B_{i,j}(t))_{i,j\in[K]})$ \Comment{$b_t$: estimated $m$-best arm at $t$} 
          
         
%          $ s_t\leftarrow \argmax_{a \in M(t)}B_{a,b_t}(t)$ \Comment{$s_t$: challenger to $b_t$ at $t$}


%          $ a_t \leftarrow$ selection\_rule$(b_t,s_t;\hat{V}_{t-1}^\lambda)$ \Comment{selecting and pulling arms}


%          $ r_t \leftarrow$ pulling$(a_t)$


%          Update $\hat{V}_t^\lambda$, $(\hat{\mu}_i(t))_{i\in[K]}$


%          Update $(B_{i,j}(t+1))_{i,j\in[K]}$

        
%          $t \gets t+1$
%    } 

%    $\hat{S}^{T_\delta}_m \leftarrow J(T_\delta)$
   
%  \textbf{Output:}
%  $\hat{S}_m^{T_\delta}$ estimated $m$ $ \epsilon$-optimal arms at final time $T_\delta$
% \end{algorithm} 





==> table-results-llms_transfer.tex <==
\begin{table}[httb]
% \footnotesize
\small
    \centering
    % \small
     % \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\textbf{Transfer}} & \multicolumn{1}{c}{\textbf{GSM8K}}& \multicolumn{1}{c}{\textbf{AquaRat}} & \multicolumn{1}{c}{\textbf{TabMWP}} & \multicolumn{1}{c}{\textbf{FinQA}}
     & \multicolumn{1}{c}{\textbf{StrategyQA}} \\
     

    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    % \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\

    \textbf{\static{}}             &  Llama2    & 77.79 & 56.30 & 83.65  & 57.72  &   82.24 \\
                             &  Mistral   & 79.91  & 54.72 & 83.42 & 59.72  & 84.49   \\
    \textbf{\static{}+\selfcon{}}     &  Llama2   & 85.67  & 63.38 & 85.08  &  63.38 &  86.93  \\
                             &  Mistral   &  86.96 & 62.20  & 84.91  & 63.64  & 87.55   \\
    \textbf{\static{}+\knn+\selfcon{}}&  Llama2    & 86.66 & 63.39 & 84.76 & 62.16 & 86.33   \\
                             &  Mistral  & 87.49 & 64.17 & 86.23 & 64.25 & 85.92   \\
    \textbf{\static{}+\mmr+\selfcon{}}&  Llama2    & 86.96   & 62.99 & 85.88 &64.43 &   85.71 \\
                             &  Mistral   &85.60  & 62.60 & 85.91 & 63.47  & 84.69   \\



     \bottomrule
    \end{tabular}
    % } 
    \caption{Results for transfer of exemplars selected using \static{} on smaller LLMs (Llama2-7b and Mistral-7b) to larger LLM (gpt-3.5-turbo).}
    % \vspace{-1cm}
    \label{tab:llm_transfer}
\end{table}







